Training Neural Speech Recognition Systems with Synthetic Speech Augmentation

Building an accurate automatic speech recognition (ASR) system requires a large dataset that contains many hours of labeled speech samples produced by a diverse set of speakers. The lack of such open free datasets is one of the main issues preventing advancements in ASR research. To address this problem, we propose to augment a natural speech dataset with synthetic speech. We train very large end-to-end neural speech recognition models using the LibriSpeech dataset augmented with synthetic speech. These new models achieve state of the art Word Error Rate (WER) for character-level based models without an external language model.

==> leftovers.tex <==
%    A key component to building a state of the art automatic speech recognition (ASR) system is the curation and processing of large datasets. The lack of such a dataset has been a key blocker in advancing ASR research. We propose a solution to this problem by creating a large synthetic dataset using a neural speech synthesis model. By combining this synthetic dataset with LibriSpeech, we train two end-to-end models that achieve state of the art word error rate performance on LibriSpeech.
    
%  One of the main problem in building large ASR systems is collecting and preparing data-sets. The lack of large free and public data-sets is one of the main blockers in the ASR research. We proposed a new approach to the building ASR systems: we generate syntetic speech out of large text dataset. Then we end-to-end train large deep learning based ASR system directly out of this synthetic speech. We build two large ASR systems which we evaluated on LibriSpeech dataset. These models reached state-of-the art accuracy WER ...    
  
  
  
%  In order to build ASR ..., one needs to have a large dataset which should contain many hours of labeled speech data produced by different speakers.

%   Training on a combined synthetic and LibriSpeech dataset allows us to get an improvement in word error rate (WER) on LibriSpeech.
   
%   By combining the synthetic dataset with LibriSpeech, we obtain an improvement in word error rate (WER) compared to training with only LibriSpeech data.
   
%   new approach to the building ASR systems: we generate syntetic speech out of large text dataset. Then we end-to-end train large deep learning based ASR system directly out of this synthetic speech. We build two large ASR systems which we evaluated on LibriSpeech dataset. These models reached state-of-the art accuracy WER ...   



\begin{itemize}
\item Wave2Letter+: fully convolutional model based on Wav2Letter \citep{collobert2016wav2letter}
\item Deep Speech 2: recurrent model \citep{Amodei2016DeepS2}
\end{itemize}
These models were trained on LibriSpeech dataset \citep{panayotov2015librispeech} that contains $\sim$1k hours of audio. WERs (word error rates) were measured on \textit{dev-clean} part of the dataset using a greedy decoder - taking at each time step the most probable character without any additional language model re-scoring.
During training in mixed-precision, we observed a total memory reduction to around 57\%, making it 3.6x faster than training using only FP32.
\begin{table}[t]
\centering
\begin{tabular}{|c|c|} 
 \hline
 \textbf{Model} & \textbf{Greedy WER (\%)}  \\
 \hline 
 Wave2Letter+ & 6.67  \\ 
  \hline 
DeepSpeech2 & 6.71  \\ 
 \hline
\end{tabular}
\caption{WERs for ASR models using mixed-precision training.}
\label{tab:wmtBLEU}
\end{table}


\subsection{Overfit with natural Librispeech dataset}

In our experiments, we trained Deep-Speech-2-like model on a ``clean'' and ``other'' subsets of LibriSpeech training dataset \citep{panayotov2015librispeech}. Table \ref{tab:table} shows final Word Error Rates (WER)\footnote{With beam width $= 2048$ and language model provided by Mozilla: \url{https://github.com/mozilla/DeepSpeech/tree/master/data/lm}} on LibriSpeech ``dev-clean'' subset, obtained after training using FP32 and mixed precision.


\subsection{Synthetic Speech  generation} 

OpenSeq2Seq supports Tacotron 2 \citep{shen2018natural} with Griffin-Lim \citep{griffin1984signal} for speech synthesis. The model currently uses only the LJ Speech dataset \citep{ito2017lj}. We plan on additionally supporting the M-AILABS dataset \citep{mailabs}. Sample audio on both datasets can be found on our documentation website\footnote{\url{https://nvidia.github.io/OpenSeq2Seq/html/speech-synthesis/tacotron-2-samples.html}}. Tacotron 2 can be trained 1.6x faster in mixed-precision compared to FP32.

